On Provable Backdoor Defense in Collaborative Learning

As collaborative learning allows joint training of a model using multiple sources of data, the security problem has been a central concern. Malicious users can upload poisoned data to prevent the model's convergence or inject hidden backdoors. The so-called backdoor attacks are especially difficult to detect since the model behaves normally on standard test data but gives wrong outputs when triggered by certain backdoor keys. Although Byzantine-tolerant training algorithms provide convergence guarantee, provable defense against backdoor attacks remains largely unsolved. Methods based on randomized smoothing can only correct a small number of corrupted pixels or labels; methods based on subset aggregation cause a severe drop in classification accuracy due to low data utilization. We propose a novel framework that generalizes existing subset aggregation methods. The framework shows that the subset selection process, a deciding factor for subset aggregation methods, can be viewed as a code design problem. We derive the theoretical bound of data utilization ratio and provide optimal code construction. Experiments on non-IID versions of MNIST and CIFAR-10 show that our method with optimal codes significantly outperforms baselines using non-overlapping partition and random selection. Additionally, integration with existing coding theory results shows that special codes can track the location of the attackers. Such capability provides new countermeasures to backdoor attacks.

==> c_additional_results.tex <==
\section{Additional results}

Here we provide some additional examples of optimal BCC codes for reference.
We perform exhaustive search to obtain all possible codes for a certain $(k,r,n)$ and then remove those codes that are equivalent up to row and column permutations.
% There is no known polynomial time algorithms of finding these codes.
\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{fig/codes.pdf}
    \caption{Optimal BRC codes obtained from exhaustive search.}
    \label{fig:codes}
\end{figure}

% The training result is summarized in Table~\ref{tab:training}, which includes the mean and standard deviations of 10 repeated runs.
% In all the cases, the attack is strong enough to produce $>99\%$ attack success rates on backdoored models (Attack-B).
% For models training on MNIST without frontend sharing, the attack success rates on clean models (Attack-C) are close to zero.
% The clean data accuracy (Clean) shows the impact of row weight $r$, where models from code 1, 4, and 6 with the highest $r$ are the most accurate.
% Due to the lack of clean training data, models from code 2, 5, and 7 with low $r$ not only suffer from low clean data accuracy, but also have a more significant ``leakage'' of the backdoor when sharing frontend networks (Attack-C on CIFAR).
% The histogram of the attack success rate is given in Figure~\ref{fig:hist}

% \begin{table}[]
% \centering
% \footnotesize
% \caption{Clean data accuracy and attack success rate on individual models before ensembling.}
% \label{tab:training}
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% Dataset &  & Code 1 & Code 2 & Code 3 & Code 4 & Code 5 & Code 6 & Code 7 \\ \midrule
% \multirow{3}{*}{MNIST} & Clean & \textbf{98.8} & 98.5 & 98.7 & \textbf{98.8} & 98.6 & \textbf{98.8} & 97.9 \\
%  & Attack-B & 98.9 & 98.8 & 98.4 & 99.4 & 98.7 & 99.3 & 91 \\
%  & Attack-C & 0.1 & 0.2 & 0.1 & 0.1 & 0.2 & 0.1 & 0.2 \\ \midrule
% \multirow{3}{*}{CIFAR} & Clean & \textbf{81.1} & 79.5 & 80 & \textbf{81.1} & 79.4 & \textbf{81.5} & 76.7 \\
%  & Attack-B & 99.6 & 99.8 & 99.7 & 99.4 & 99.6 & 99.5 & 99.7 \\
%  & Attack-C & 4.3 & \textbf{14.2} & 6.8 & 5.3 & \textbf{7.5} & 3.0 & \textbf{12.1} \\ \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{fig/histogram.pdf}
%     \caption{Attack success rate on backdoored models and clean models before decoding.}
%     \label{fig:hist}
% \end{figure}
